A High-Performance Triple Patterning Layout Decomposer with Balanced Density

Triple patterning lithography (TPL) has received more and more attentions from industry as one of the leading candidate for 14nm/11nm nodes. In this paper, we propose a high performance layout decomposer for TPL. Density balancing is seamlessly integrated into all key steps in our TPL layout decomposition, including density-balanced semi-definite programming (SDP), density-based mapping, and density-balanced graph simplification. Our new TPL decomposer can obtain high performance even compared to previous state-of-the-art layout decomposers which are not balanced-density aware, e.g., by Yu et al. (ICCAD'11), Fang et al. (DAC'12), and Kuang et al. (DAC'13). Furthermore, the balanced-density version of our decomposer can provide more balanced density which leads to less edge placement error (EPE), while the conflict and stitch numbers are still very comparable to our non-balanced-density baseline.

==> doc/app_example.tex <==
%\vspace{-.1in}
\section{Decomposition Example}
\label{sec:app_example}




==> doc/app_proof.tex <==


\vspace{-.1in}
\section{Proof of Lemmas}
\label{sec:app_proof}







==> doc/app_result.tex <==

\vspace{-.1in}
\section{Additional Experimental Results}
\label{sec:app_result}


%\begin{itemize}
%  \item {benchmark statistics}
%\end{itemize}
                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 


==> doc/app_sdp.tex <==
%\vspace{-.1in}
\appendix
\label{sec:app}

\iffalse
% Table of Notations
%{{{
\begin{table}[thb]
\vspace{-.1in}
\renewcommand{\arraystretch}{1}
\centering
\caption{Notations used in this paper}
\label{table:app_notation}
\begin{tabular}{|c|c|}
    \hline \hline
    %\multicolumn{2}{|c|}{Notations used in Mathematical programming}\\
    %\hline
    $CE$          & the set of conflict edges\\
    \hline
    $SE$          & the set of stitch edges\\
    \hline
    $V$           & the set of features\\
    \hline
    $r_i$         & the $i_{th}$ layout feature\\
    \hline
    $len_i$       & the density of $r_i$\\
    \hline
    $x_i$         & variable denoting the color (mask) of $r_i$\\
    \hline
    $c_{ij}$      & 0-1 variable, $c_{ij}=1$ if conflict between $r_i$ and $r_j$\\
    \hline
    $s_{ij}$      & 0-1 variable, $s_{ij}=1$ if stitch between $r_i$ and $r_j$\\
    \hline\hline
\end{tabular}
\vspace{-.1in}
\end{table}
%}}}
\fi

%The basic formulation of our vector programming is similar to that in \cite{TPL_ICCAD2011_Yu}:
In this section we discuss some preliminary for the semidefinite programming (SDP).
In TPL layout decomposition, three unit vectors are used to represent three different masks (colors).
Each vertex is associated with one of three unit vectors:
$(1, 0)$, $(-\frac{1}{2}$, $\frac{\sqrt{3}}{2})$ and $(-\frac{1}{2}, -\frac{\sqrt{3}}{2})$.
Note that the angle between any two vectors of the same mask is $0$, while the angle between vectors with different masks is $2\pi/3$.
Additionally, from the inner product for any two unit vectors $\vec{v_i}, \vec{v_j}$, we get the following property:
\begin{displaymath}
    \vec{v_i} \cdot \vec{v_j} =
    \left\{
    \begin{array}{cc}
        1,          & \vec{v_i} = \vec{v_j}\\
        -\frac{1}{2}    & \vec{v_i} \ne \vec{v_j}
    \end{array}
    \right.
  \label{eq:vivj}
\end{displaymath}

%Given the stitch candidates, the decomposition graphs construction is carried out.
For each decomposition graph, a mathematical formulation can be generated to minimize the cost of stitch and conflict.
In \cite{TPL_ICCAD2011_Yu} semidefinite programming (SDP) is presented to provide an approximate solution to the mathematical formulation.
\begin{align}
    \textrm{SDP:\ \ min}    & \ \ \ A \bullet X                     \notag\\
                & X_{ii} = 1,              \ \ \forall i \in V         \tag{$a$}\\
                & X_{ij} \ge -\frac{1}{2}, \ \ \forall e_{ij} \in CE   \tag{$b$}\\
                & X \succeq 0                                          \tag{$c$}\label{sdp_old_c}
\end{align}
where $A \bullet X$ is an inner product between two matrices $A$ and $X$, i.e., $\sum_i \sum_j A_{ij}X_{ij}$.
Here $A_{ij}$ is the entry that lies in the $i$-th row and the $j$-th column of matrix $A$.
\begin{equation}
    A_{ij} =
    \left\{
    \begin{array}{cc}
        1,               & \forall e_{ij} \in CE\\
        -\alpha,         & \forall e_{ij} \in SE\\
        0,               & \textrm{otherwise}
    \end{array}
    \right. \notag
\label{eq:a}
\end{equation}

The above SDP formulation can be solved in polynomial time, and the results are stored in a matrix $X$.
Ideally, we hope $X_{ij}$ in the matrix $X$ to be distinguishable (either close to $1$ or $-0.5$).
For each $X_{ij}$, if it is close to $1$, vertices $r_i$ and $r_j$ tend to be in the same color (mask);
while if it is close to $-0.5$, $r_i$ and $r_j$ tend to be in different colors (masks).
%Our preliminary results show that with reasonable threshold such as $0.9 < X_{ij} \le 1$ for same color, and $-0.5 \le X_{ij} < -0.4$ for different colors,
%more than 80\% of vertices can be decided by the global SDP optimization.
However, SDP only provides an approximation solution to the mathematical formulation, therefore some $X_{ij}$ values may be not so distinguishable.




==> doc/app_stitch.tex <==

\vspace{-.1in}
\section{Stitch Candidate Generation}
\label{sec:app_stitch}

Stitch candidate generation is one important step to parse a layout.
%It not only determines the vertex number in the decomposition graph, but also affects the decomposition result.
%\cite{DPL_ICCAD09_Xu}\cite{DPL_ICCAD08_Kahng} propose different methodologies to generate the DPL candidates.
%We use \textit{DPL candidates} to represent the stitch candidates generated by double patterning (DPL) problem.
\cite{TPL_DAC2012_Fang}\cite{TPL_SPIE2011_Ghaida} pointed out that the stitch candidates generated by previous DPL  works cannot be directly applied in TPL layout decomposition.
Therefore, we provide a procedure to generate appropriate stitch candidates for TPL.
The main idea is that after projection, each feature is divided into several segments each of which is labeled with a number representing how many other features are projected onto it.
If one segment is projected by less than two features, then a stitch can be introduced.
Note that to reduce the problem size, we restrict the maximum stitch candidate number on each feature.




==> doc/cover.tex <==

\twocolumn[
\normalsize
\begin{@twocolumnfalse}

Dear ICCAD Technical Program Chair,

\ \\
We are submitting this article as the camera-­‐ready version of ICCAD’13.

In the following, we summarize the differences between this version and the previously submitted version.

\begin{itemize}
  \item
  {
    We included authors, affiliation, and acknowledgment.
  }
  \item
  {
    We changed the font size from 10pt to 9pt, so the page number is changed to 7.
  }
  \item
  {
    We released new version of our layout decomposer, and updated the related experimental result tables.
  }
  \item
  {
    Add references: [2][14]
  }
  \item
  {
    Typos have been corrected:
    \begin{itemize}
      \item
      {
        [In abstract]: ``... by Yu et al. (ICCAD'11) and Fang et al. (DAC'12).
        Specifically, a 65-81\% decrease in the weighted sum of the conflicts and stitches can be achieved.''
        $\rightarrow$
        ``... by Yu et al. (ICCAD'11), Fang et al. (DAC'12), and Kuang et al. (DAC'13).''
      }
      \item
      {
        [In conclusion]: ``... and fast color assignment trial and graph simplifications''
        $\rightarrow$
        ``... and fast color assignment trial''.
      }
    \end{itemize}
  }
\end{itemize}

Thank you.

\ \\
Best regards,

\ \\
Bei Yu, Yen-Hung Lin, Gerard Luk-Pat, Duo Ding, Kevin Lucas, David Z. Pan

\end{@twocolumnfalse}
]



==> doc/flow.tex <==




==> doc/old/SDP.tex <==
\section{Density Balanced Decomposition}
\label{sec:algo_db}

Compared with the traditional time consuming integer linear programming (ILP),
semidefinite programming (SDP) has been shown to be a better approach for the TPL layout decomposition in terms of runtime and solution quality tradeoff \cite{TPL_ICCAD2011_Yu}.
However, how to integrate the density balance issue into the formulation is still an open question.
In this section, we show that using a novel transformation, the density balance can be accurately integrated into the vector programming and the corresponding SDP.
Besides, several graph based methods considering density balance will be discussed.
Because of all these methods, the density balancing can be taken into account in each step of the decomposition flow.


\subsection{Density Balanced Mathematical Formulation}
%/*{{{*/

The mathematical formulation for the density balanced TPL layout decomposition is shown in (\ref{eq:math}).
The objective of (\ref{eq:math}) is to simultaneously minimize the conflict number, the stitch number and the density balance value $DB$.
$\alpha$ and $\beta$ are user-defined parameters for assigning the relative weights among the three values.

\begin{align}
  \footnotesize
  \label{eq:math}
  \textrm{min}      &   \sum_{e_{ij} \in CE} c_{ij} + \alpha \sum_{e_{ij} \in SE}s_{ij} + \beta \cdot DB & \\
  \textrm{s.t}.\ \
    & c_{ij} = ( x_i == x_j )                       &\forall e_{ij} \in CE      \label{1a}\tag{$1a$}\\
    & s_{ij} = x_i \oplus x_j                       &\forall e_{ij} \in SE      \label{1b}\tag{$1b$}\\
    & x_i \in \{0, 1, 2\}                             &\forall r_i \in V        \label{1c}\tag{$1c$}\\
    & d_k = \sum_{x_i = k} len_i                  &\forall r_i \in V        \label{1d}\tag{$1d$}\\
    & DB = \textrm{max}\{d_k\} / \textrm{min}\{d_k\}                        \label{1e}\tag{$1e$}
\end{align}

Here $x_i$ is a variable representing the color (mask) of feature $r_i$, $c_{ij}$ is a binary variable for the conflict edge $e_{ij} \in CE$, and $s_{ij}$ is a binary variable for  the stitch edge $e_{ij} \in SE$.
The constraint (\ref{1a}) is used to evaluate the conflict number when the touched vertices $r_i$ and $r_j$ are assigned different masks.
The constraint (\ref{1b}) is used to calculate the stitch number. If vertices $r_i$ and $r_j$ are assigned the same mask, the stitch $s_{ij}$ is introduced.

The constraint (\ref{1e}) is nonlinear, which makes the program (\ref{eq:math}) hard to be formulated into ILP like in \cite{TPL_ICCAD2011_Yu}.
Similar nonlinear constraints occur in the floorplanning problem \cite{FLOOR_DAC00_Chen}, where Tayor expansion was used to linearize the constraint into ILP.
However, Tayor expansion will introduce the penalty of accuracy.
In the following section we show that instead of using the painful Tayor expansion, this nonlinear constraint can be integrated into a vector program without losing any accuracy.
%/*}}}*/


\subsection{Density Balanced Vector Programming}
%/*{{{*/

%The basic formulation of our vector programming is similar to that in \cite{TPL_ICCAD2011_Yu}:
We use three unit vectors to represent three different masks.
Each vertex is associated with one of three unit vectors:
$(1, 0), (-\frac{1}{2}, \frac{\sqrt{3}}{2})$ and $(-\frac{1}{2}, -\frac{\sqrt{3}}{2})$.
Note that the angle between any two vectors of the same mask is $0$, while the angle between vectors with different masks is $2\pi/3$.
Additionally, from the inner product for any two unit vectors $\vec{v_i}, \vec{v_j}$, we get the following property:
\begin{equation}
    \vec{v_i} \cdot \vec{v_j} =
    \left\{
    \begin{array}{cc}
        1,          & \vec{v_i} = \vec{v_j}\\
        -\frac{1}{2}    & \vec{v_i} \ne \vec{v_j}
    \end{array}
    \right.
  \label{eq:vivj}
\end{equation}

\cite{TPL_ICCAD2011_Yu} shows that without the nonlinear constraint (\ref{1e}), the program (\ref{eq:math}) can be formulated into a vector programming,
where the objective function is the representation of the vector inner products, i.e., $\vec{v_i} \cdot \vec{v_j}$.
At the first glance, the constraint (\ref{1e}) cannot be formulated into an inner product format.
However, we show that density balance value $DB$ has a special relationship with $DB_2$ as follows:
\begin{displaymath}
  DB_2 = d_1 \cdot d_2 + d_1 \cdot d_3 + d_2 \cdot d_3
\end{displaymath}

\begin{lemma}
Maximizing $DB_2$ is equivalent to minimizing $DB$. \label{lem:1}
\end{lemma}

The proof of lemma \ref{lem:1} is provided in Appendix \ref{chap:app_proof}.
Since maximizing $DB_2$ is equivalent to minimizing $DB$, if $DB_2$ can be formulated as a representation of vector inner products,
then we find a way to integrate the constraint (\ref{1e}) into the vector program.


\begin{lemma}
$DB_2 = 2/3 \cdot \sum_{i, j \in V} len_i \cdot len_j \cdot (1 - \vec{v_i} \cdot \vec{v_j})$
\label{lem:2}
\end{lemma}

Here the $len_i$ is the density of feature $r_i$.
The proof of lemma \ref{lem:2} is given in Appendix \ref{chap:app_proof}.
Combining Lemma \ref{lem:1} and Lemma \ref{lem:2}, we have proved the
following theorem.

\begin{theorem}
Maximizing $DB_2$ can achieve a better density balance.
\end{theorem}

Note that the expression $\sum_{i,j \in V} len_i \cdot len_j \cdot 1$ in $DB_2$ is a constant,
and we can replace $DB_2$ with $DB_2^*$ by removing the constant part.
Similarly, we can eliminate the constants in the calculation of the conflict and stitch numbers.
The simplified vector program is as follows:

\begin{align}
  \small
  \label{eq:vp}
  \textrm{min}  & \sum_{e_{ij} \in CE} ( \vec{v_i} \cdot \vec{v_j} ) - \alpha \sum_{e_{ij} \in SE} ( \vec{v_i} \cdot \vec{v_j} ) - \beta \cdot DB_2^*\\
  \textrm{s.t}.\ \
    & DB_2^* = - \sum_{i, j \in V} len_i \cdot len_j \cdot ( \vec{v_i} \cdot \vec{v_j})                       \label{3a}\tag{$3a$}\\
    & \vec{v_i} \in \{(1, 0), (-\frac{1}{2}, \frac{\sqrt{3}}{2}), (-\frac{1}{2}, -\frac{\sqrt{3}}{2})\}     \label{3b}\tag{$3b$}
\end{align}

%/*}}}*/


\subsection{Density Balanced SDP Approximation}
%/*{{{*/

Formulation (\ref{eq:vp}) is equivalent to the mathematical formulation (\ref{eq:math}), and it is still NP-hard to be solved exactly.
Constraint (\ref{3b}) requires the solutions to be discrete.
To achieve a good tradeoff of runtime and accuracy, we relax constraint (\ref{3b}) to generate formula (\ref{eq:sdp}) as following:

\begin{align}
  \vspace{-.1in}
  \label{eq:sdp}
  \textrm{min}  & \sum_{e_{ij} \in CE} ( \vec{y_i} \cdot \vec{y_j}) - \alpha \sum_{e_{ij} \in SE} ( \vec{y_i} \cdot \vec{y_j} ) - \beta \cdot DB_2^*\\
  \textrm{s.t}.\ \
    & DB_2^* = - \sum_{i, j \in V} len_i \cdot len_j \cdot (\vec{y_i} \cdot \vec{y_j})    \label{sdpa}\tag{$4a$}\\
    & \vec{y_i} \cdot \vec{y_i} = 1 ,               \ \ \ \forall i \in V                   \label{sdpb}\tag{$4b$}\\
    & \vec{y_i} \cdot \vec{y_j} \ge -\frac{1}{2},   \ \ \ \forall e_{ij} \in CE             \label{sdpc}\tag{$4c$}
\end{align}

Here each unit vector $\vec{v_i}$ is replaced by a $n$ dimensional vector $\vec{y_i}$.
The solution of (\ref{eq:sdp}) is continuous instead of discrete, and provides a lower bound of vector program (\ref{eq:vp}).
In other words, (\ref{eq:sdp}) provides an approximated solution to (\ref{eq:vp}).
To solve program (\ref{eq:sdp}) in polynomial time, we show that it can be represented as the following standard SDP:

\begin{align}
    \label{eq:sdp2}
    \textrm{SDP:\ \ min}    & \ \ \ A \bullet X                     \\
                & X_{ii} = 1,              \ \ \forall i \in V                  \tag{$5a$}\\
                & X_{ij} \ge -\frac{1}{2}, \ \ \forall e_{ij} \in CE        \tag{$5b$}\\
                & X \succeq 0                                                             \label{sdp2c}\tag{$5c$}
\end{align}
where $A \bullet X$ is an inner product between two matrices $A$ and $X$, i.e., $\sum_i \sum_j A_{ij}X_{ij}$.
Here $A_{ij}$ is the entry that lies in the $i$-th row and the $j$-th column of matrix $A$.
\begin{displaymath}
    A_{ij} =
    \left\{
    \begin{array}{cc}
        1 + \beta \cdot len_i \cdot len_j,               & \forall e_{ij} \in CE\\
        -\alpha + \beta \cdot len_i \cdot len_j,         & \forall e_{ij} \in SE\\
        \beta \cdot len_i \cdot len_j,                   & \textrm{otherwise}
    \end{array}
    \right.
\end{displaymath}
The constraint (\ref{sdp2c}) means that the matrix $X$ should be positive semidefinite.
SDP (\ref{eq:sdp2}) can be solved in polynomial time, and the
results are stored in a matrix $X$. Each $X_{ij}$ in the matrix $X$
represents $\vec{y_i} \cdot \vec{y_j}$, which is an approximation of
$\vec{v_i} \cdot \vec{v_j}$. Because of the property (\ref{eq:vivj}), ideally we
hope $X_{ij}$ can be distinguishable (either close to $1$ or
$-0.5$). However, SDP (\ref{eq:sdp2}) only provides an approximation
solution to the vector program.
%We can take advantage of $X_{ij}$ as a guideline for the color assignment.
For each $X_{ij}$, if it is close to $1$, vertices $r_i$ and $r_j$ tend to be in the
same color (mask); while if it is close to $-0.5$, $r_i$ and $r_j$
tend to be in different colors (masks). Our preliminary results show
that with reasonable threshold such as $0.9 < X_{ij} \le 1$ for same
color, and $-0.5 \le X_{ij} < -0.4$ for different colors, more than
80\% of vertices can be decided by the global SDP optimization.
%For those $X_{ij}$ not so clear, we propose a mapping process to search the final color assignment.
%but sometimes $X_{ij}$ is not so clear, especially when there are some conflicts.

%/*}}}*/


==> doc/old/mapping.tex <==

\subsection{Density Balanced Mapping}
\label{sec:mapping}
%{{{

As discussed above, each $X_{ij}$ in solution of (\ref{eq:sdp2}) provides a guideline, i.e., whether $r_i$ and $r_j$ should be in same color.
With these guidelines a mapping procedure is adopted to finally assign all vertices into three colors (masks).
In \cite{TPL_ICCAD2011_Yu}, a greedy approach was applied for this color assignment.
The idea is straightforward: $X_{ij}$s are sorted, and vertices $r_i$ and $r_j$ with larger $X_{ij}$ value tend to be in the same color.
If most of the $X_{ij}$s in matrix $X$ are clear (close to 1 or -0.5), this greedy method may achieve good result.
However, if the decomposition graph is not 3-colorable, some values in matrix $X$ are vague.
For these vague $X_{ij}$, e.g., 0.5, the greedy method is not so effective.

Different from previous greedy approach, we propose a density balanced mapping, which is based on a three-way partitioning.
The main ideas are as follows. All $X_{ij}$s are classified into two types: clear and vague.
If a $X_{ij}$ is clear, the relationship of vertices $r_i$ and $r_j$ can be directly decided.
For those vague $X_{ij}$s, instead of only relying on the SDP solution, we also take advantage of the information in decomposition graph.
These information are captured in a graph construction.
Followed by a three-way partitioning on this graph, our mapping can provide a global view to search solutions.
In addition, density balance can be naturally integrated into the partitioning,
and therefore our mapping can provide more balanced decomposed results.


\begin{algorithm}[thb]
\caption{Density Balanced Mapping}
\label{alg:mapping}
\begin{algorithmic}[1]
   \REQUIRE Solution matrix $X$ of the program (\ref{eq:sdp2}).
   \STATE Label each non-zero entry $X_{i, j}$ as a triplet $(X_{ij}, i, j)$;
   \STATE Sort all $(X_{ij}, i, j)$ by $X_{ij}$;
   \FOR { all triples with $X_{ij} > th_{unn}$}
      \STATE Union(i, j);
   \ENDFOR
   \FOR { all triples with $X_{ij} < th_{sp}$}
      \STATE Separate(i, j);
   \ENDFOR
   \STATE Construct graph;
   \IF{graph size $\le$ 3}
      \STATE return;
   \ELSIF{graph size $\le 7$}
      \STATE Backtracking based three-way partitioning;
   \ELSE
      \STATE FM based three-way partitioning;
   \ENDIF
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:mapping} shows our density balanced mapping procedure.
Given the solutions from program (\ref{eq:sdp2}), some triplets are constructed and sorted to maintain all non-zero $X_{ij}$ values (lines 1--2).
Then the mapping incorporates two stages to deal with the two different types.

The first stage (lines 3--8) is similar to that in \cite{TPL_ICCAD2011_Yu}.
If $X_{ij}$ is clear then the relationship between vertices $r_i$ and $r_j$ can be directly determined.
Here $th_{unn}$ and $th_{sp}$ are user-defined threshold values.
%They determine what kind of $X_{ij}$ belongs to the clear type.
For example, if $X_{ij} > th_{unn}$, which means that $r_i$ and $r_j$ should be in the same color,
then function Union(i, j) is applied to merge them into a large vertex.
Similarly, if $X_{ij} < th_{sp}$, then function Separate(i, j) is used to label $r_i$ and $r_j$ as incompatible.
If $r_i$ and $r_j$ are incompatible, they cannot be merged and function Compatible(i, j) will return $false$.

In the second stage (lines 9--16) we deal with the vague $X_{ij}$s.
%<CLARIFICATION: can you give an estimate on "not large" in terms of starting size? as in, G is the set of all groups, and |G| ~= 10% |V| or something?>
During the first stage some vertices have been merged, therefore the total vertex number is not large.
Here we construct a graph to represent the relationships among all the remanent vertices (line 9).
Each edge $e_{ij}$ in this graph has a weight representing the cost if vertices $i$ and $j$ are assigned into a same color.
Therefore, the color assignment problem can be formulated as a maximum-cut partitioning problem on this graph (line 10--16).
Note that the graph can further consider density balance by adding a weight on each vertex to represent its density.

% Here is an example
An example of the graph construction and maximum-cut partitioning is shown in Fig. \ref{fig:mapping}.
Based on the decomposition graph (see Fig. \ref{fig:mapping} (a)), SDP is formulated.
Given the solutions of SDP, after the first stage, vertices $a_2$ and $d_2$ are merged in to a large vertex $A$,
while other four vertices are un-merged.
Then a new graph is constructed as in Fig. \ref{fig:mapping} (b).
Each edge is associated with a value representing the cost of assigning those vertices the same color.
To consider the density balance, each vertex has a weight as its density.
A partitioning is performed on this graph to simultaneously search a max-cut and balance weight among different parts.
There are two partition results with the same cut value (see Fig. \ref{fig:mapping} (c) and Fig. \ref{fig:mapping} (d)).
Their density balance values are 24 and 23, respectively.
To keep a more balanced density result, the second partitioning is adopted.
Corresponding color assignment result is shown in Fig. \ref{fig:mapping} (e).

%\begin{define}[Group Graph]
%The group graph is an undirected graph whose vertices are the group vertices.
%An edge exists if and only if there are conflict edges or stitch edges between the two group vertices.
%\end{define}

\begin{figure}[tb]
    \centering
    \subfigure[]{
        \includegraphics[width=0.15\textwidth]{DAC_ex5}
    }
    \hspace{-.1in}
    \subfigure[]{
        \includegraphics[width=0.15\textwidth]{GroupGraph1}
    }
    \hspace{-.1in}
    \subfigure[]{
        \includegraphics[width=0.15\textwidth]{GroupGraph2}
    }
    \subfigure[]{
        \includegraphics[width=0.15\textwidth]{GroupGraph3}
    }
    \subfigure[]{
        \includegraphics[width=0.15\textwidth]{DAC_ex6}
    }
    \nocaptionrule
    \caption{~(a) Decomposition graph.~(b) Graph construction for three-way maximum-cut partitioning.
    ~(c) One partitioning result with cut value 8.1 and DB 24.
    ~(d) A better result with cut 8.1 and DB 23.
    ~(e) Final color assignment result.}
    \label{fig:mapping}
    \addtolength{\belowcaptionskip}{-5mm}
\end{figure}



It is well known that the maximum-cut problem, even for a 2-way partition, is NP-hard.
However, we observe that in lots of cases, after the global SDP optimization, the partitioning problem size could be quite small, i.e., less than 7.
For these small problems, we apply a backtracking based method to search entire solution space.
Note that for these small problems backtracking can quickly find the optimal solution even three-way partitioning is NP-hard.
If the graph size is larger, we propose a heuristic method, motivated by the classic FM partitioning algorithm
\cite{PAR_DAC82_FM}\cite{PAR_TC89_Sanchis}.
Different from the classic FM partitioning algorithm, we make the following modifications.
(1) In the first stage some vertices are labeled as incomparable, therefore before moving a vertex from one partition to another,
we should check whether it is legal.
(2) Different from the traditional min-cut partition, we modify the gain function of each move to achieve a maximum cut.
(3) Density balance value is considered in the gain function.
In other words, in each move, we try to achieve a balanced density.


\iffalse
Here an important concept is called the ``vertex move".
%Each vertex has a gain value showing how much cut can be increased if it is moved from current partition to another one.
At every move, the vertex who can achieve the most cut increasing is
chosen to move from current partition to another one. Another
important concept is called the ``pass", where all vertices are
moved exactly once during a single pass. When a vertex is chosen to
move because it has the maximum cut increasing, we move it even when
the increasing value is negative. At the end of the current pass, we
accept the first $K$ movings that lead to the best partition, which
may contain some not so good movings.
\fi

% ************************************
%       Runtime analyse
% ************************************
The Disjoint-set data structure is used to implement functions
Union() and Separate(). Under a special implementation, the running
time of each function can be almost constant \cite{book90Algorithm}.
Let $n$ be the number of vertices and the number of triplets is
$O(n^2)$. Sorting all the triplets requires $O(n^2logn)$. The
runtime complexity of graph construction is $O(m)$, where $m$ is the
number of vertices. The runtime of three-way maximum-cut
partitioning algorithm is $O(m logm)$. Since $m$ is much smaller
than $n$, then the complexity of density balanced mapping is
$O(n^2logn)$.
%}}}


\vspace{-.1in}
\subsection{Density Balanced Graph Simplification}
In previous we have discussed the color assignment for the decomposition graphs.
It shall be noted that the problem size can be dramatically simplified through graph simplification
\cite{TPL_ICCAD2011_Yu}\cite{TPL_DAC2012_Fang}.
In this subsection, we further discuss some techniques not only speed up the computation of decomposition,
but also keep a better density balancing.

\vspace{-.05in}
\subsubsection{Density Balanced Iterative Vertex Recover}
Motivated by the work in \cite{TPL_ICCAD2011_Yu}, we iteratively
remove and push all vertices with degree less than or equal to two.
After the color assignment on the remained vertices, we iteratively recover all the removed vertices and assign legal colors.
Instead of randomly assigning a legal color, we assign one legal color which is good to the density balance.

\vspace{-.05in}
\subsubsection{Density Balanced Decomposition Graph Merging}
Using independent component computation and bridge computation \cite{TPL_ICCAD2011_Yu}\cite{TPL_DAC2012_Fang}, the whole design can be broken down into several components.
After color assignment independently on each component, all the color assignment results are merged together.
Note that two components share almost one edge or one vertex,
then we can rotate the colors in one component so that merging introduces no more stitch or conflict.
Besides, there is no cycle when we merge the decomposition graphs, the merging can be done in linear time through a
breadth-first search (BFS).

\vspace{-.05in}
\subsubsection{Color Assignment for Simple Decomposition Graph}
Through the layout graph simplification \cite{TPL_ICCAD2011_Yu}, for each vertex in the layout graph, its degree is larger than or equal to 2.
However, after introducing the stitch edges and the bridge computation, corresponding decomposition graphs would have some differences.
For each decomposition graph, we first iteratively remove the vertex with degree less than 3.
If the whole decomposition graph can be removed, the color assignment is completed in linear time.
Otherwise, we recover the vertices and apply SDP based color assignment as discussed above.
Our preliminary results show that lots of decomposition graphs can be decomposed using this fast method.
By this way, the runtime can be further reduced.


==> doc/old/motivation.tex <==

\vspace{-.1in}
\section{Motivation and Preliminaries}
\label{sec:motivation}

% *****************************************************
%                     Motivation
% *****************************************************
\vspace{-.05in}
\subsection{Motivation}

\begin{figure}[bht]
    \centering
    \includegraphics[width=0.4\textwidth]{UnbalancedLayout}
    \nocaptionrule
    \caption{~***Need new aerial image for triple patterning case.
    Unbalanced decomposition may cause some disconnections.}
    \label{fig:aerial}
    \addtolength{\belowcaptionskip}{-3mm}
\end{figure}

In the previous section we discussed the need for a systematic methodology to consider the density balance in the layout
decomposition.
In this section, we use an example to further motivate such requirement.
Even though two features within minimum space are assigned to different masks, unbalanced density can cause
lithography hotspots as well as lowered CD uniformity due to
irregular pitch. The aerial image of an unbalanced decomposition can
have a patterning problem as shown in Fig. \ref{fig:aerial}.
%The balanced decomposition of the same circuit in Fig. \ref{fig:aerial}(b) does not have the problem.
Even though the decomposed layout in Fig. \ref{fig:aerial} does not
represent a general case, balanced decomposition provides more
lithography friendly layout because of higher regularity
\cite{DPL_ASPDAC2010_Yang}.
Therefore, balanced density should be considered in the decomposition problem.

\subsection{Layout Graph and Decomposition Graph}

\begin{figure}[bht]
    \centering
    \subfigure[]{
        \includegraphics[width=0.12\textwidth]{DAC_DG1}
    }
    \subfigure[]{
        \includegraphics[width=0.12\textwidth]{DAC_DG2}
    }
    \subfigure[]{
        \includegraphics[width=0.12\textwidth]{DAC_DG3}
    }
  \nocaptionrule
    \caption{~(a) Input layout.~(b) Layout graph, where all edges are conflict edges.~(c) Decomposition graph after the stitch candidate generation, where dash edges denote stitch edges.}
    \label{fig:graphs}
\end{figure}

Our layout decomposition is carried out on graph representations.
As shown in Fig. \ref{fig:graphs}, after getting an input layout we construct the layout graph and the decomposition graph.
In the layout graph each vertex represents a polygonal feature (shape) where there is an edge (conflict edge) between two vertices if and only if those two vertices are within the minimum coloring distance $min_s$.
The decomposition graph maintains all the information about conflict edges and stitch candidates.
For example, in Fig. \ref{fig:graphs} (c) the solid edges are the conflict edges while the dashed edges are the stitch edges and function as stitch candidates.




==> doc/old/stitch.tex <==

\vspace{-.1in}
\section{Stitch Candidate Generation}
\label{sec:stitch}

Stitch candidate generation is one of the most important steps to parse the layout.
It not only determines the vertex number in the decomposition graph, but also affects the decomposed result.
%\cite{DPL_ICCAD09_Xu}\cite{DPL_ICCAD08_Kahng} propose different methodologies to generate the DPL candidates.
We use \textit{DPL candidates} to represent the stitch candidates generated by all previous DPL research.
\cite{TPL_ICCAD2011_Yu} directly applies these DPL candidates in the TPL layout decomposition.
In this section, we show that since DPL stitch candidates may be redundant or lose some useful candidates,
they cannot be directly used in TPL layout decomposition.
Furthermore, we provide a procedure to generate appropriate stitch candidates for TPL.
%Note that our update methodology can be easily extended to generate stitch candidates from scratch.



% *********************************************************************
%           Redundant and Lost Stich
% *********************************************************************
\subsection{Redundant Stitch and Lost Stitch}


\begin{figure}[htb]
  \vspace{-.1in}
  \centering
  \subfigure[]{
    \includegraphics[width=0.18\textwidth]{RedundantStitch1}
  }
  \subfigure[]{
    \includegraphics[width=0.2\textwidth]{LostStitch1}
  }
  \nocaptionrule
  \caption{~(a) Redundant stitch.~(b) This stitch cannot be detected in the DPL stitch candidate generation.}
  \label{fig:DPL_Stitch}
  \addtolength{\belowcaptionskip}{-3mm}
\end{figure}

We provide several examples to demonstrate why DPL candidates are not appropriate for TPL.
First, because of an extra color choice, some DPL candidates may be redundant.
As shown in Fig. \ref{fig:DPL_Stitch} (a), the stitch can be removed because no matter how to assign colors for the features $b$ and $c$,
the feature $a$ can always be assigned a legal color.
We denote this kind of stitch as a \textit{redundant stitch}.
After removing these redundant stitches, some extra vertices in the decomposition graph can be merged.
In this way, we can reduce the problem size.
Besides, some useful stitch candidates cannot be detected during previous DPL stitch candidate generation.
In DPL, the stitch candidate has one precondition: it cannot intersect with any projection.
For example, as shown in Fig. \ref{fig:DPL_Stitch} (b),
because this stitch intersects with the projection of feature $b$, it cannot belong to the DPL candidates.
However, if features $b, c$ and $d$ are assigned with three different colors, only introducing this stitch can resolve the conflict.
In other words, the precondition in DPL limits the ability of stitches to resolve the triple patterning conflicts and may result in unnoticed conflicts.
We denote the useful stitches forbidden by the DPL precondition as a \textit{lost stitch}.



% *********************************************************************
%           Stitch Candidate Update
% *********************************************************************
\subsection{Stitch Candidate Generation}
Given the projection results, we carry out stitch candidate generation.
As discussed above, compared with the DPL stitches, in TPL the redundant stitches need to be removed and some lost stitches should be added.
%Our generation process is based on projection sequence.
For a better explanation, let us define the projection sequence.

\begin{define}[Projection Sequence]
After the projection, the feature is divided into several segments each of which is labeled with a number representing how many other features are projected onto it.
The sequence of numbers on these segments is the projection sequence.
\end{define}

\begin{figure}[htb]
\vspace{-.1in}
  \centering
  \includegraphics[width=0.35\textwidth]{ProjectNum}
  \nocaptionrule
  \caption{~The projection sequence of the feature is $01212101010$, and the last $0$ is a default terminal zero.}
  \label{fig:projectNum}
  \addtolength{\belowcaptionskip}{-3mm}
\end{figure}

Instead of analyzing each feature and its all neighbor features, we can directly carry out stitch candidate generation based on the projection sequence.
For convenience, we provide a terminal zero rule, i.e., the beginning and the ending of the projection sequence must be $0$.
To maintain this rule, sometimes a default $0$ needs to be added at the end of sequence.
For example, in Fig. \ref{fig:projectNum}, the middle feature has five conflict features $b, c, d, e$ and $f$.
Based on the projection results, the feature is divided into ten segments.
Through labeling each segment, we can get its projection sequence: $01212101010$.
Here a default $0$ is added at the end of the feature.

Based on the definition of projection sequence, we summarize the rule for redundant stitches and lost stitches.
First, motivated by the case in Fig. \ref{fig:DPL_Stitch} (a), we can summarize the redundant stitches as follows:
if the projection sequence begins with ``$01010$", then the first stitch candidate in DPL is redundant.
Since the projection of a feature can be symmetric, if the projection sequence ends with ``$01010$", then the last stitch candidate is also redundant.
%Note that we can not detect all the redundant stitches before really coloring.
Besides, the rule for lost stitches is as follows.
if a projection sequence contains the sub-sequence ``$xyz$", where $x, y, z > 0$ and $x>y, z>y$, then there is one lost stitch at the segment labeled as $y$.
For example, the stitch candidate in Fig. \ref{fig:DPL_Stitch} (b) is contained in the sub-sequence ``$212$", so it is a lost stitch.


The details of stitch candidate generation are shown in Algorithm \ref{alg:stitch}.
If necessary, at first each multiple-pin feature is decomposed into several two-pin features.
Then for each feature, we calculate its projection sequence.
We remove the redundant stitches by checking if the projection sequence begins or ends with ``$01010$".
Next we search for and insert the lost stitches.
Here we define a \textit{sequence bunch}.
A sequence bunch is a sub-sequence of a projection sequence, and contains at least three non-$0$ segments.
%Inside each two $0$s there is at most one sequence bunch.
For simplicity, in our algorithm to identify the lost stitch candidate, at most one stitch is introduced between two $0$s for each sequence bunch.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.45\textwidth]{StitchGeneration}
  \nocaptionrule
  \caption{~Stitch candidates generated for DPL and TPL.}
  \label{fig:stitch}
  \addtolength{\belowcaptionskip}{-3mm}
\end{figure}


\begin{algorithm}[htb]
\caption{Stitch Candidate Generation}
\label{alg:stitch}
\begin{algorithmic}[1]
  \REQUIRE Projection results on features.
  \STATE Decompose multiple-pin features;
  \FOR { each feature $w_i$}
    \STATE Calculate the projection sequence $ps_i$;
    \IF{$ps_i$ begins or ends with ``$01010$"}
      \STATE Remove redundant stitch(es);
    \ENDIF
    \FOR { each sequence bunch of $ps_i$ }
      \STATE Search and insert at most one lost stitch candidate;
    \ENDFOR
  \ENDFOR
\end{algorithmic}
\end{algorithm}


An example of the stitch candidate generation is shown in Fig. \ref{fig:stitch}.
Using the DPL stitch candidate generation, there are two stitch candidates generated by the DPL methodology (stitch 2 and stitch 3).
Through our rule for TPL stitch candidate, stitch 3 is labeled as a redundant stitch.
Besides, stitch 1 is identified as a lost stitch candidate because it is located in a sub-sequence ``$212$".
Therefore, stitch 1 and stitch 2 are chosen as stitch candidates for TPL.


==> doc/others.tex <==



==> doc/stitch.tex <==

\vspace{-.1in}
\section{Stitch Candidate Generation}
%{{{

Stitch candidate generation is one of the most important steps to parse a layout.
It not only determines the vertex number in the decomposition graph, but also affects the decomposition result.
%\cite{DPL_ICCAD09_Xu}\cite{DPL_ICCAD08_Kahng} propose different methodologies to generate the DPL candidates.
We use \textit{DPL candidates} to represent the stitch candidates generated by all previous DPL research.
In this section, we show that since DPL candidates may be redundant or lose some useful candidates,
they cannot be directly applied in TPL layout decomposition.
Therefore, we provide a procedure to generate appropriate stitch candidates for TPL.

\vspace{-.1in}
\subsection{Limitations of DPL Candidates}

\begin{figure}[htb]
  \vspace{-.1in}
  \centering
  \subfigure[]{
    \includegraphics[width=0.18\textwidth]{RedundantStitch1}
  }
  \subfigure[]{
    \includegraphics[width=0.2\textwidth]{LostStitch1}
  }
  \caption{~(a) Redundant stitch.~(b) This stitch cannot be detected in the DPL candidate generation.}
  \label{fig:DPL_Stitch}
  \vspace{-.1in}
\end{figure}

We provide two examples to demonstrate why DPL candidates are not appropriate for TPL.
First, because of an extra color choice, some DPL candidates may be redundant.
As shown in Fig. \ref{fig:DPL_Stitch} (a), the stitch can be removed because no matter what color is assigned to features $b$ and $c$,
the feature $a$ can always be assigned a legal color.
We denote this kind of stitch as a \textit{redundant stitch}.
After removing these redundant stitches, some extra vertices in the decomposition graph can be merged.
In this way, we can reduce the problem size.
Besides, DPL candidates may cause the stitch loss problem, i.e., some useful stitch candidates cannot be detected and inserted in layout decomposition.
In DPL, the stitch candidate has one precondition: it cannot intersect with any projection.
For example, as shown in Fig. \ref{fig:DPL_Stitch} (b),
because this stitch intersects with the projection of feature $b$, it cannot belong to the DPL candidates.
However, if features $b, c$ and $d$ are assigned with three different colors, only introducing this stitch can resolve the conflict.
In other words, the precondition in DPL limits the ability of stitches to resolve the triple patterning conflicts and may result in unnoticed conflicts.
We denote the useful stitches forbidden by the DPL precondition as a \textit{lost stitch}.

\cite{TPL_ICCAD2011_Yu} directly applies the DPL candidates, which limit their ability to search better solutions.
Although in \cite{TPL_DAC2012_Fang} the stitch insertion followed by color assignment may overcome the stitch loss problem,
their post-stage process suffers from unnecessary stitch penalty.

\vspace{-.1in}
\subsection{Stitch Candidate Generation for TPL}

Given the projection results, we propose a new stitch candidate generation.
Compared with the DPL candidates, our methodology can remove some redundant stitches and systematically solve the stitch loss problem.
%Our generation process is based on projection sequence.
For a better explanation, let us define the projection sequence.

\begin{mydefinition}[Projection Sequence]
After the projection, the feature is divided into several segments each of which is labeled with a number representing how many other features are projected onto it.
The sequence of numbers on these segments is the projection sequence.
\end{mydefinition}

\begin{figure}[htb]
\vspace{-.1in}
  \centering
  \includegraphics[width=0.35\textwidth]{ProjectNum}
  \caption{~The projection sequence of the feature is $01212101010$, and the last $0$ is a default terminal zero.}
  \label{fig:projectNum}
  \vspace{-.1in}
\end{figure}

Instead of analyzing each feature and all its neighboring features, we can directly carry out stitch candidate generation based on the projection sequence.
For convenience, we provide a terminal zero rule, i.e., the beginning and the end of the projection sequence must be $0$.
To maintain this rule, sometimes a default $0$ needs to be added.
An example of projection sequence is shown in Fig. \ref{fig:projectNum}, where the middle feature has five conflict features, $b, c, d, e$ and $f$.
Based on the projection results, the feature is divided into ten segments.
Through labeling each segment, we can get its projection sequence: $01212101010$.
Here a default $0$ is added at the end of the feature.

Based on the definition of projection sequence, we summarize the rules for redundant stitches and lost stitches.
First, motivated by the case in Fig. \ref{fig:DPL_Stitch} (a), we can summarize the redundant stitches as follows:
if the projection sequence begins with ``$01010$", then the first stitch in DPL candidates is redundant.
Since the projection of a feature can be symmetric, if the projection sequence ends with ``$01010$", then the last stitch candidate is also redundant.
%Note that we can not detect all the redundant stitches before really coloring.
Besides, the rule for lost stitches is as follows,
if a projection sequence contains the sub-sequence ``$xyz$", where $x, y, z > 0$ and $x>y, z>y$, then there is one lost stitch at the segment labeled as $y$.
For example, the stitch candidate in Fig. \ref{fig:DPL_Stitch} (b) is contained in the sub-sequence ``$212$", so it is a lost stitch.


The details of stitch candidate generation for TPL are shown in Algorithm \ref{alg:stitch}.
If necessary, at first each multiple-pin feature is decomposed into several two-pin features.
Then for each feature, we can calculate its projection sequence.
We remove the redundant stitches by checking if the projection sequence begins or ends with ``$01010$".
Next we search for and insert stitches, including the lost stitches.
Here we define a \textit{sequence bunch}.
A sequence bunch is a sub-sequence of a projection sequence, and contains at least three non-$0$ segments.
%Inside each two $0$s there is at most one sequence bunch.
For simplicity, in our algorithm to identify the lost stitch candidate, at most one stitch is introduced between two $0$s for each sequence bunch.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.45\textwidth]{StitchGeneration}
  \caption{~Stitch candidates generated for DPL and TPL.}
  \label{fig:stitch}
  \vspace{-.1in}
\end{figure}


\begin{algorithm}[htb]
\caption{Stitch Candidate Generation for TPL}
\label{alg:stitch}
\begin{algorithmic}[1]
  \REQUIRE Projection results on features.
  \STATE Decompose multiple-pin features;
  \FOR { each feature $w_i$}
    \STATE Calculate the projection sequence $ps_i$;
    \IF{$ps_i$ begins or ends with ``$01010$"}
      \STATE Remove redundant stitch(es);
    \ENDIF
    \FOR { each sequence bunch of $ps_i$ }
      \STATE Search and insert at most one stitch candidate;
    \ENDFOR
  \ENDFOR
\end{algorithmic}
\end{algorithm}


An example of the stitch candidate generation is shown in Fig. \ref{fig:stitch}.
In the DPL candidate generation, there are two stitch candidates generated (stitch 2 and stitch 3).
Through our stitch candidate generation, stitch 3 is labeled as a redundant stitch.
Besides, stitch 1 is identified as a lost stitch candidate because it is located in a sub-sequence ``$212$".
Therefore, stitch 1 and stitch 2 are chosen as stitch candidates for TPL.

%}}}



